A Fixed-Target Programme at the LHC: Physics Case and Projected Performances for Heavy-Ion, Hadron, Spin and Astroparticle Studies

We review the context, the motivations and the expected performances of a comprehensive and ambitious fixed-target program using the multi-TeV proton and ion LHC beams. We also provide a detailed account of the different possible technical implementations ranging from an internal wire target to a full dedicated beam line extracted with a bent crystal. The possibilities offered by the use of the ALICE and LHCb detectors in the fixed-target mode are also reviewed.

==> detector/buffer <==
\subsubsection{Comparison of possible implementations}

\begin{figure}[hbt!]
\centering
\includegraphics[width=0.6\textwidth]{detector/expAcceptanceReview.pdf}
\caption{Centre-of-mass-rapidity (\ycms) coverage as a function of the colliding energies per nucleon pair 
(\sqrtsNN) as in \cf{fig:acceptance}. The blue lines represent the acceptance of the TPC and MS 
of ALICE. The full, long-dashed and short-dashed 
lines correspond to targets located at the IP, upstream of the IP, at $z_{\rm target}$ = -2.75 and -4.7 m, 
respectively. The dash-dotted green lines represent the acceptance of the LHCb detector with a target 
at the IP and the dash-triple-dotted green lines with a target upstream of the IP by $z_{\rm target}=1.5$~m. 
The long-dashed and short-dashed blue lines as well as the dash-dotted and dash-triple-dotted green lines are shifted in energy 
for a better visibility. 
}
\label{fig:acceptanceComparison-FTLHC}
\end{figure}

\cf{fig:acceptanceComparison-FTLHC} shows the \ycms acceptances of the 
ALICE and LHCb detectors for two fixed-target energies, namely $\sqrtsNN = 72$ GeV and 115 GeV. The rapidity coverages with a 
target position at the nominal IP are shown as full line for ALICE and dash-dotted line for LHCb. 
The latter corresponds to the case of LHCb used as a fixed-target detector
with the SMOG system. The acceptances are also shown with two (one) other target positions for ALICE (LHCb), where the acceptance is determined considering the geometry of the active part of the detector as detailed in Section~\ref{section:detector:alice} and ~\ref{section:detector_lhcb}. For a target located at the IP, the 
ALICE MS and the LHCb detectors cover the central \ycms region as well as 
half of the backward rapidity acceptance ($\ycms<0$), while the ALICE CB has the particularity to probe the target-rapidity region and 
the end of the phase space ($x_2 \to 1$ and $x_F \to -1$). When the target is shifted on the opposite side of the detector, the rapidity interval probed is shifted forward. In the ALICE and LHCb cases, the wide \ycms range makes these detectors suitable 
to study the rapidity dependence of various probes. 

\begin{table}[!hbt]
\center
\begin{adjustbox}{angle=90}
%\resizebox{0.89\textheight}{!}{
\renewcommand{\arraystretch}{1.2}
\begin{tabularx}{0.87\textheight}{p{1.5cm}|c|c|c|c|c|c|c|c|c|c}
%\begin{tabularx}{0.87\textheight}{p{1.5cm}|p{1.2cm}|p{1.9cm}|c|c|p{1cm}|c|c|c|p{.8cm}|c}
%\multicolumn{3}{|c}{ } & \multicolumn{6}{|c|}{Beam} \\
%\cline{4-9}
%\multicolumn{3}{|c}{ } & \multicolumn{4}{|c|}{ALICE} & \multicolumn{4}{c|}{ LHCb} \\
\multicolumn{3}{c}{ } & \multicolumn{8}{|c}{ALICE}  \\
\multicolumn{3}{c}{ } & \multicolumn{4}{|c|}{Proton beam (\sqrtsNN = 115 GeV)} & \multicolumn{4}{c}{Pb beam (\sqrtsNN = 72 GeV)} \\
\cline{4-11}
\multicolumn{3}{c|}{Target} & $\cal L$ & $\sigma_{inel.}$  & $\Gamma_{inel.}$ &   $\int\cal L$ &  $\cal L$   & $\sigma_{inel.}$  & $\Gamma_{inel.}$  & $\int\cal L$ \\
\multicolumn{3}{c|}{} & [cm$^{-2}$ s$^{-1}$] & [mb]  &  [kHz] & [pb$^{-1}$]  & [cm$^{-2}$ s$^{-1}$] & [b] &   [kHz] & [nb$^{-1}$]  \\

\hline
\hline
\multirow{9}{*}{\parbox{1.5cm}{\centering Internal gas target}} %& \multirow{1}{*}{SMOG} & He, Ne, Ar & 5.8 $\times 10^{29}$   & 0.25 $\times 10^{6}$  & 145 & 7.4 $\times 10^{25}$  & 10$^{6}$  & 0.074   \\
								%	\cline{2-9}
								%	& SMOG++ &  Xe, Ne, Ar, He, Kr &  &  &  &   && \\
								%	\cline{2-3}
								    &\multirow{4}{*}{\centering Gas-Jet} & H$^\uparrow$  &  4.3 $\times 10^{30}$  & 39  & 168  & 43   &  5.6 $\times 10^{26}$  & 1.8 & 1.0  & 5.6 $\times 10^{-1}$  \\
								    	&							   & H$_{2}$ & 2.6 $\times 10^{31}$   &  39 & 1000 & 2.6 $\times 10^{2}$ & 2.8 $\times 10^{28}$   & 1.8 & 50  & 28  \\
									&							   & D$^\uparrow$ & 4.3 $\times 10^{30}$   & 72 & 309  & 43 & 5.6 $\times 10^{26}$  & 2.2 & 1.2 & 5.6 $\times 10^{-1}$  \\
									&							   & $^3$He$^\uparrow$ & 8.5 $\times 10^{30}$   & 117  & 1000  & 85 & 2.0 $\times 10^{28}$  & 2.5 & 50 & 20 \\
&							  									   & Xe &  7.7 $\times 10^{29}$  & 1300 & 1000  &  7.7   &  8.1 $\times 10^{27}$ & 6.2  & 50  &   8.1   \\
							     	\cline{2-11}
									&\multirow{5}{*}{\parbox{1.5cm}{\centering Storage Cell}} & H$^\uparrow$  & 2.6 $\times 10^{31}$   &  39 & 1000 & 2.6 $\times 10^{2}$ & 2.8 $\times 10^{28}$   & 1.8 & 50  & 28  \\
									&							   & H$_{2}$  & 2.6 $\times 10^{31}$   &  39 & 1000 & 2.6 $\times 10^{2}$ & 2.8 $\times 10^{28}$   & 1.8 & 50  & 28  \\  
									&							   & D$^\uparrow$ & 1.4 $\times 10^{31}$  &  72 & 1000   & 1.4 $\times 10^{2}$  & 2.2 $\times 10^{28}$  & 2.2  &  50 & 22  \\
									&							   & $^3$He$^\uparrow$ & 8.5 $\times 10^{30}$   & 117  & 1000  & 85 & 2.0 $\times 10^{28}$  & 2.5 & 50 & 20 \\
									&							   & Xe &  7.7 $\times 10^{29}$  & 1300  & 1000  & 7.7   & 8.1 $\times 10^{27}$ & 6.2  & 50  &  8.1   \\ \hline
\multirow{3}{*}{\parbox{1.5cm}{\centering Internal solid target on beam halo}}& \multirow{4}{*}{\parbox{1.2cm}{\centering Wire Target}} & C (500 $\mu$m) & 2.8 $\times 10^{30}$ & 271   & 760  & 28  & 5.6 $\times 10^{26}$ & 3.3 & 1.8 & 5.6 $\times 10^{-1}$ \\
								&		      & Ti (500 $\mu$m) &  1.4 $\times 10^{30}$   &  694 & 971 & 14  & 2.8 $\times 10^{26}$  & 4.7 & 1.3  &  2.8 $\times 10^{-1}$  \\			
									                                                 &	          & W (184 $\mu$m) &   5.9  $\times 10^{29}$ & 1700  & 1000  & 5.9  & --& -- & --& --  \\	
                            &	          & W (500 $\mu$m) & --   & --  & -- & -- & 3.1 $\times 10^{26}$ & 6.9  & 2.1 & 3.1 $\times 10^{-1}$ \\		\hline
\multirow{6}{*}{\parbox{1.5cm}{\centering Beam splitting}}& \multirow{2}{*}{\centering E1039} & NH$_3^\uparrow$ & 2.4 $\times 10^{30}$   &  420 & 1000 & 24  & 2.7 $\times 10^{27}$  &  19 & 50 & 2.7  \\
							   &  &  ND$_3^\uparrow$ & 1.9 $\times 10^{30}$ & 519  & 1000  &  19 & 2.2 $\times 10^{27}$  & 22 & 50 & 2.2 \\
							%   &  & $ND_3$  &  &  &  &  &&  \\
							%   &  & He &  &  &  &  &&  \\
						     	\cline{2-11}
						     	             &   & C (658 $\mu$m ) & 3.7 $\times 10^{30}$ & 271  & 1000 & 37  & --& -- & -- & -- \\
          &   & C (5 mm) & --  & -- & -- & -- & 5.6 $\times 10^{27}$ & 3.3 & 18 & 5.6  \\
									&			\multirow{3}{*}{\parbox{1.2cm}{\centering Unpol\-arised solid target}}				                                              & Ti (515 $\mu$m) &  1.4 $\times 10^{30}$  & 694  & 1000 & 14  & --  & -- & -- &  -- \\	
&							                                              & Ti (5 mm) &  --  &-- & -- & -- & 2.8 $\times 10^{27}$  & 4.7 & 13 &  2.8 \\	
									&							                                              & W(184 $\mu$m) &   5.9  $\times 10^{29}$ & 1700  & 1000  & 5.9 & -- & --  & - & --    \\ 
& & W(5 mm) &   -- & -- & --  & -- & 3.1 $\times 10^{27}$ & 6.9  & 21 & 3.1 \\ \hline
\end{tabularx} 
%}
\end{adjustbox}
\caption{Summary table of the achievable integrated luminosities with the ALICE detector accounting for the data-taking-rate capabilities in the collider mode and by considering the luminosities of \ct{tab_lumi_comp}. As detailed in the text, a higher inelastic rate ($\Gamma_{inel.}$) depending on the collision system could be envisioned. The inelastic cross sections ($\sigma_{inel.}$) are taken from EPOS~\cite{Pierog:2013ria,Werner:2005jf}.}							
\label{tab_lumi_comp_alice}
\end{table}

\flushfootnote

\ct{tab_lumi_comp_alice} and \ct{tab_lumi_comp_lhcb} 
show the achievable luminosities using the ALICE and LHCb detectors during one LHC year, if one considers as a limitation
the aforementioned experimental data-taking rates in the collider mode and by considering the luminosities of \ct{tab_lumi_comp}. 
As specified in Section~\ref{section:detector:alice}, a higher rate could be envisioned in some cases since the charged-particle multiplicity 
is lower in the fixed-target mode.  
We have also assumed that ALICE and LHCb could run in the fixed-target mode during the full year with proton ($10^7$~s) and lead beams ($10^6$~s) with the corresponding instantaneous luminosities. 
In some cases, namely the gas-jet, the storage-cell and the solid target coupled to the beam splitting by a crystal, the resulting interaction rates are
high and close to those expected in the collider mode for the LHC Runs 3 and 4. Additional limitations will arise from
various constraints such as the disk storage, the high-level trigger, the radiation level, the simultaneous running with the collider mode, etc. The Run 3 and Run 4 programmes for ALICE and LHCb are well settled in the collider mode and any fixed-target-running scenario will have to comply with these programmes. These 
constraints are not discussed in this review as they deserve dedicated studies within the experiments. In the following, we discuss the luminosities obtained with the three technical implementations in both the ALICE and LHCb set-ups and comment on the luminosity needs for some of the physics cases that will be described in sections~\ref{section:High-x}, \ref{section:Spin-Physics} and \ref{section:heavy Ion Physics}. 

\begin{table}[!hbt]
\center
\begin{adjustbox}{angle=90}
%\resizebox{0.9\textheight}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabularx}{0.9\textheight}{p{2.0cm}|c|c|c|c|c|c|c|c|c|c}
%\multicolumn{3}{|c}{ } & \multicolumn{6}{|c|}{Beam} \\
%\cline{4-9}
%\multicolumn{3}{|c}{ } & \multicolumn{4}{|c|}{ALICE} & \multicolumn{4}{c|}{ LHCb} \\
\multicolumn{3}{c}{ } & \multicolumn{8}{|c}{LHCb}  \\
\multicolumn{3}{c}{ } & \multicolumn{4}{|c|}{Proton beam (\sqrtsNN = 115 GeV)} & \multicolumn{4}{c}{Pb beam (\sqrtsNN = 72 GeV)} \\
\cline{4-11}
\multicolumn{3}{c|}{Target } & $\cal L$  & $\sigma_{\rm inel.}$  & $\Gamma_{inel.}$ &  $\int\cal L$ & $\cal L$  & $\sigma_{\rm inel.}$  & $\Gamma_{inel.}$  & $\int\cal L$  \\
\multicolumn{3}{c|}{} & [cm$^{-2}$ s$^{-1}$] & [mb]  &  [kHz] & [pb$^{-1}$]  & [cm$^{-2}$ s$^{-1}$] & [mb] &   [kHz] & [nb$^{-1}$]  \\
\hline
\hline
   %& \multirow{1}{*}{SMOG} & He, Ne, Ar & 5.8 $\times 10^{29}$   & 0.25 $\times 10^{6}$  & 145 & 7.4 $\times 10^{25}$  & 10$^{6}$  & 0.074   \\
								%	\cline{2-9}
								%	& SMOG++ &  Xe, Ne, Ar, He, Kr &  &  &  &   && \\
								%	\cline{2-3}
		\multirow{10}{*}{\parbox{2cm}{\centering Internal	gas target}	}						    &\multirow{5}{*}{\centering Gas-Jet}  & H$^\uparrow$  &  4.3 $\times 10^{30}$  & 39  & 168  & 43   &  5.6 $\times 10^{26}$  & 1.8 & 1  & 5.6 $\times 10^{-1}$ \\
								    	&							   & H$_{2}$ & 1.0 $\times 10^{33}$  & 39  & 40000  & 1.0 $\times 10^4$  & 1.2 $\times 10^{29}$  & 1.8 & 212  & 1.2 $\times 10^{2}$  \\
									&							   & D$^\uparrow$ &  4.3 $\times 10^{30}$  & 72 & 309  & 43  & 5.6 $\times 10^{26}$  & 2.2 & 1 & 5.6 $\times 10^{-1}$  \\
									&							   & $^3$He$^\uparrow$ & 3.4 $\times 10^{32}$  & 117  &  40000 & 3.4 $\times 10^3$  & 4.7 $\times 10^{28}$ & 2.5 & 118  & 47  \\
&							  									 & Xe &  3.1 $\times 10^{31}$  & 1300  & 40000 & 3.1 $\times 10^{2}$  & 2.3 $\times 10^{28}$  & 6.2 & 186 &  23 \\
							     	\cline{2-11}
							&\multirow{5}{*}{\parbox{1.5cm}{\centering Storage Cell}} & H$^\uparrow$ & 9.2 $\times 10^{32}$  & 39 & 35880 & 9.2 $\times 10^3$   & 1.2 $\times 10^{29}$  & 1.8 & 212 & 1.2 $\times 10^{2}$ \\
									&							   & H$_{2}$ &  1.0 $\times 10^{33}$   & 39 & 40000 & 1.0$\times 10^4$  & 1.2 $\times 10^{29}$  & 1.8 & 212 & 1.2 $\times 10^{2}$ \\
									&							   & D$^\uparrow$ & 5.6 $\times 10^{32}$   & 72  & 40000  & 5.6 $\times 10^3$   & 8.8 $\times 10^{28}$  & 2.2 & 194 & 88  \\
									&							   & $^3$He$^\uparrow$ & 1.3 $\times 10^{33}$ & 117  & 40000  & 1.3 $\times 10^4$ & 8.3 $\times 10^{28}$  & 2.5 & 206 & 83 \\
									&							   & Xe & 3.1 $\times 10^{31}$  & 1300  & 40000 & 3.1 $\times 10^{2}$ & 3.0 $\times 10^{28}$  & 6.2 & 186 &  30 \\
\hline
\multirow{3}{*}{\parbox{2cm}{\centering Internal solid target on beam halo}}  & \multirow{3}{*}{\parbox{1.2cm}{\centering Wire Target}} & C (500 $\mu$m) &  2.8 $\times 10^{30}$ & 271   & 760  & 28   & 5.6 $\times 10^{26}$ & 3.3  & 2 & 5.6 $\times 10^{-1}$\\
 	&							                   & Ti (500 $\mu$m) &  1.4 $\times 10^{30}$ & 694  & 972  & 14   & 2.8 $\times 10^{26}$  & 4.7 & 1  &  2.8 $\times 10^{-1}$  \\				
								&							                                & W (500 $\mu$m) &  1.6 $\times 10^{30}$ &  1700 & 2720  & 16    & 3.1 $\times 10^{26}$ & 6.9  & 2 & 3.1 $\times 10^{-1}$  \\		\hline
\multirow{5}{*}{\parbox{1.5cm}{\centering Beam splitting}}& \multirow{2}{*}{\centering E1039} & NH$_3^\uparrow$ & 7.2 $\times 10^{31}$ & 420 & 30240 & 7.2 $\times 10^{2}$  & 1.4 $\times 10^{28}$  &  19 & 259 & 14  \\
							   &  &  ND$_3^\uparrow$ & 7.2 $\times 10^{31}$ & 519  & 37368  & 7.2 $\times 10^{2}$  & 1.4 $\times 10^{28}$  & 22 & 314 & 14 \\
							%   &  & $ND_3$  &  &  &  &  &&  \\
							%   &  & He &  &  &  &  &&  \\
						     	\cline{2-11}
						     	             & \multirow{3}{*}{\parbox{1.2cm}{\centering Unpol\-arised solid target}}   & C (5 mm) &  2.8 $\times 10^{31}$ & 271  & 7600  & 2.8 $\times 10^{2}$ & 5.6 $\times 10^{27}$ & 3.3 & 18 & 5.6  \\
									&			 				                             				  & Ti (5 mm)  &  1.4 $\times 10^{31}$ & 694  & 9720  & 1.4 $\times 10^{2}$ & 2.8 $\times 10^{27}$  & 4.7 & 13 &  2.8 \\		
									&							                                               & W (5 mm) &  1.6 $\times 10^{31}$ &  1700 & 27200  & 1.6 $\times 10^{2}$ & 3.1 $\times 10^{27}$ & 6.9 & 21 & 3.1    \\ \hline
\end{tabularx} 
%}
\end{adjustbox}
\caption{Same as \ct{tab_lumi_comp_alice} for the LHCb detector.}							
\label{tab_lumi_comp_lhcb}
\end{table}

With LHCb, the luminosity reach with a proton beam on an hydrogen target can be very large, up to yearly luminosity of the order of $10$~fb$^{-1}$, if one can run at 40~MHz for a full LHC year. As discussed in section~\ref{section:High-x}, this will allow one to measure hard probes such as $W$ or associated \jpsi production, to collect very large statistics for DY and probe the $D$ meson production at the most backward rapidity range. For example, DY measurements are very useful to probe the light quark and anti-quark PDFs at high-$x$ and a low scale, $\mu_F$, even with a reduced luminosity of $1$~fb$^{-1}$. By using nuclear solid or gas targets, one can reach luminosities on the order of 100~pb$^{-1}$, and even more depending on the target option, allowing one to probe the nuclear PDFs with a very high precision by measuring DY, open heavy flavour and quarkonium production. 
With proton and lead beams, the luminosity reach for ALICE is lower than for LHCb because of the lower data-taking rates. However, the rapidity coverage is complementary as well as the physics reach. Even though with ALICE the yearly luminosity can be as high as $250$~pb$^{-1}$ with a proton beam on a H-gas target, a luminosity of about $40$~pb$^{-1}$ with the ALICE detectors 
would already allow one to measure low energy $\bar p$, thanks to the very backward rapidity coverage, in $p+p \to \bar p + X$. This measurement would improve our knowledge of the cosmic $\bar p$ spectrum. The $\bar p$ spectrum could be further measured with various target types, such as He or C with the gas or solid target option, respectively.  

With a transversally polarised H-gas target, luminosities from about $40$~pb$^{-1}$ to $250$~pb$^{-1}$ can be expected with ALICE for one LHC year. As discussed in section~\ref{section:Spin-Physics}, this would allow one to access the spin asymmetry of probes such as $\Lambda$ in the CB and \jpsi in the MS. With a larger luminosity in LHCb, on the order of $10$~fb$^{-1}$, similar rare probes as those mentioned above for the unpolarised case ($W$, associated \jpsi, DY, ...) will be accessible. These studies will definitely advance our understanding of the internal spin structure of the proton and neutron.

 With a Pb beam on a heavy nuclear target, the luminosity is mainly limited by the impact on the beam lifetime for the gas target and by the usable beam flux for the beam splitting case. The luminosities do not differ by more than a factor of four between ALICE (${\cal L}=8$~nb$^{-1}$) and LHCb (${\cal L}=30$~nb$^{-1}$) for \PbXe. In the case of the beam splitting option, large luminosities are also expected (${\cal L}= 3$~nb$^{-1}$) for \PbW.  When the nuclear target is lighter,  the Pb beam lifetime is less affected and the luminosities are larger for the case of LHCb coupled to a gas target. 
A full programme of heavy-ion studies can be carried out in the fixed-target mode at the LHC in particular with precise quarkonium measurements, with studies of the heavy-quark energy-loss mechanism and a rapidity scan of the yield and elliptic flow of identified charged particles over a broad rapidity range, as discussed in section~\ref{section:heavy Ion Physics}. These studies can be performed with large statistics in PbA collisions but also in \pp and \pA collisions (see \eg\ \ct{tab:Upsilon_yields} for the $\Upsilon$ case), with the ALICE and LHCb detectors. In the latter case, it is not yet established up to which event centrality the tracks can efficiently be reconstructed, in particular for the heaviest nuclear target such as Xe. As discussed in section~\ref{section:detector_lhcb}, on-going studies will give more information on the event-centrality reach with LHCb for the Run~3 and Run~4. A heavy-ion programme is already envisioned in LHCb in Run 3 with Ar gas target that will allow one to study soft probes as well as hard probes such as open heavy flavour and quarkonium production. 



==> motivation/buffer <==
\section{Motivations} \label{sec:motivations}

%\EditorialComment{
%relatively short info (up to 5-6 pages ) about compelling physics open questions which could be addressed with fixed target experiment with LHC beams.
%}


%\PastedText{JPL}{comments-07Jun16.txt}{
%[Have a look at the introduction of the HPH proposal to refresh one's memory about catchy sentences]\\
%\\
%Main ideas which should be addressed in this intro: \\
%$\to$ Why do we do spin physics, high-x physics, and heavy-ion physics? \\
%$\to$ Even more general than the physics punchline \\ 
%$\to$ Description of open questions with some pictures \\
%\\
%- Make a short list of 5-10 fundamental quantities that we want to address:\\
%\\
%- Origin of nucleon spin \\
%- Phase Diagram of nuclear matter\\
%- Equation of state of QGP / Phase transition of nuclear matter / viscosity\\
%- Nucleon content at large momentum (link with confinement)\\
%- Nuclear effects (find a concept) / quark gluon content of the nuclei \\
%- Cosmic Neutrino flux $\to$ Charm  \\
%- Gluon luminosity $\to$ BSM physics \\
%- EMC effect? \\
%\\
%Tentative list of figures: \\
%- Fig1 : How the spins of the building blocks of matter add up $\to$ interesting if we connect it with the TMDs  \\
%- Spin decomposition (Equation or shown a pie diagram)\\
%- Q2 vs x diagram with marked regions where AFTER could contribute\\
%\\
%( A side comment: to make the context sound more general, let us make reference to "standard model" rather than to "QCD")\\
%}


%\PastedText{JPL}{Punchline on Googledocs}{
%Punchline:\\ 
%Very large uncertainties above x~0.5. \\
%Essential QCD baseline for all high-mass BSM searches at the LHC. \\
%Proton (intrinsic) charm content is essential for the interpretation of high-energy neutrino and cosmic-rays physics \\
%Understanding the EMC effect (depletion of large-x partons) in the nucleus. Open problem since the 80s \\
%Search of gluonic protons where the gluon carry most of the momentum of the proton \\
%Essential baseline to interpret the partonic level of nuclei and initial conditions of quark-gluon plasma formation 
%}



\input{motivation/motivation-high-x.tex}

\input{motivation/motivation-spin.tex}

\input{motivation/motivation-heavy-ion.tex}


==> physics-heavy-ion-collisions/buffer <==



In this context, we find it useful to start by discussing the unique reach of \AFTER\ for $\Upsilon(nS)$ production in \pp, \pA\ and \AA\ collisions as a function of the system size (for various colliding systems or vs. collision centrality), \pt\ and rapidity, in \PbA\ collisions at $\sqrt{s_{NN}} =$ 72 GeV. This lies nearly half way between the SPS and RHIC energy ranges and significantly lower than the only existing studies by CMS at the (collider mode) LHC~\cite{Sirunyan:2017lzi,Khachatryan:2016xxp,Chatrchyan:2012lxa}.
Although the relative suppression of the $\Upsilon(nS)$ cannot  readily be used as a thermometer it will bring crucial new inputs for our understanding of the nature of the hot medium created in this energy range as opposed to that presently available at the LHC.


\begin{figure}[hbt!]
\centering
\begin{tabular}{ll}
\subfigure[~]{\includegraphics[width=0.45\textwidth]{physics-heavy-ion-collisions/UpsilonStates72gev_BkgFit_Xe_UpsilonSignal_pt7y3-5.pdf}\label{fig:Upsilon_HI:mass}} &
\subfigure[~]{\includegraphics[width=0.53\textwidth]{physics-heavy-ion-collisions/Ups_R_PbXe-080618.pdf}\label{fig:Upsilon_HI:RAA}} \\
\end{tabular}
	\caption{(a) The $\Upsilon(nS)$ signal after the (like-sign) uncorrelated-background subtraction with the expected statistical uncertainties in \PbXe collisions at $\sqrt{s_{NN}} =$ 72 GeV in the $\Upsilon$ acceptance range of 3 $< Y^{\rm lab}_{\mu\mu} < $ 5, for a LHCb-like detector. No nuclear modifications are assumed, $\mathcal L_{\rm PbXe}$ = 30 nb$^{-1}$. (b) Statistical-uncertainty projections for measurements of the nuclear modification factors \RPbXe\ and \RpXe~\cite{Trzeciak:2017csa}. The uncertainties are calculated using the yields given in \ct{tab:Upsilon_yields}.}
\label{fig:Upsilon_HI}
\end{figure}

%\begin{comment}
\begin{table}[!htb]
\begin{center}
{\renewcommand{\arraystretch}{1.5}
\subtable{\begin{tabular}{c|c|c}
%\hline
 $\Upsilon(1S)$ & $S$ & $S/B$ \\ \hline \hline
\pp & 1.33 $\times 10^{3}$ & 29.0 \\ 
\pXe & 1.39 $\times 10^{3}$ & 7.8 \\
 \PbXe & 4.33 $\times 10^{3}$ & 1.8 $\times 10^{-1}$ \\ \hline
\end{tabular}}
\subtable{\begin{tabular}{c|c|c}
$\Upsilon(2S)$  & $S$ & $S/B$ \\ \hline \hline
\pp & 2.92 $\times 10^{2}$ & 8.2 \\ %\cline{2-4}
\pXe & 3.06 $\times 10^{2}$ & 2.2 \\
\PbXe & 9.56 $\times 10^{2}$ & 5.0 $\times 10^{-2}$ \\ \hline
\end{tabular}}
\subtable{\begin{tabular}{c|c|c}
$\Upsilon(3S)$  & $S$ & $S/B$ \\ \hline \hline
\pp & 1.37 $\times 10^{2}$ & 10.3 \\ %\cline{2-4}
\pXe & 1.44 $\times 10^{2}$ & 2.8 \\
\PbXe & 4.49 $\times 10^{2}$ & 6.2 $\times 10^{-2}$ \\ \hline
\end{tabular}}}
\end{center}
\caption{$\Upsilon(nS)$ signal yields ($S$) and signal-over-combinatorial-background ratios ($S/B$) for \pp, \pXe and \PbXe collisions at $\sqrt{s_{NN}} = 72$~GeV and $3 < y_{\rm Lab.} <  5$ assuming LHCb-like performances~\cite{Trzeciak:2017csa} with $\int \mathcal L_{pp} = 250\, {\rm pb}^{-1}$, $\int \mathcal L_{p{\rm Xe}} = 2\, {\rm pb}^{-1}$ and $\int \mathcal L_{\rm PbXe} = 30\, {\rm nb}^{-1}$.}
\label{tab:Upsilon_yields}
\end{table}
%\end{comment}


\cf{fig:Upsilon_HI:mass} shows the di-muon invariant-mass distribution in the $\Upsilon(nS)$ mass range for a single year of  data taking with a LHCb-like setup.
The expected \ups\ yields are clearly large enough with the excellent resolution of LHCb to clearly distinguish each $\Upsilon(nS)$ state
in an energy domain where \ups\ studies are extremely demanding. The yields together with the signal over background ratios in \pp, \pXe\ and \PbXe\ collisions are also gathered in Table~\ref{tab:Upsilon_yields}. Projections of the statistical precision of the nuclear modification factors for the $\Upsilon(nS)$ states measured in \pXe\ and \PbXe\ collisions are presented in \cf{fig:Upsilon_HI:RAA}. The statistical uncertainties take into account the background subtraction procedure using the like-sign method. If needed, this can further be improved by using the mixed-event technique. The predictions do not include potential modifications of the $\Upsilon(nS)$ yields due to the nuclear effects. 

\begin{figure}[hbt!]
	\centering
	\includegraphics[width=0.6\textwidth]{physics-heavy-ion-collisions/Comovers-Rups-vs-energy.pdf}
	\caption{The relative suppression of the excited $\Upsilon(nS)$ states to the $\Upsilon(1S)$ as a function of the energy in iCIM~\cite{Ferreiro:2018wbd}.}
	\label{fig:R:Upsilon_comovers}
\end{figure}


\cf{fig:R:Upsilon_comovers} shows the expected relative suppression $R_{\Upsilon(nS)/\Upsilon(1S)}$\footnote{
The relative suppression R is defined as the double ratio of excited $\Upsilon$ states to the $\Upsilon(1S)$ in \AA\ and \pp\ collisions, $R_{\Upsilon(nS)/\Upsilon(1S)} = [\Upsilon(nS)/\Upsilon(1S)]_{AA}/[\Upsilon(nS)/\Upsilon(1S)]_{pp}$~\cite{Chatrchyan:2011pe,Sirunyan:2017lzi}.} in the improved Comover Interaction Model (iCIM) recently applied to describe the $\Upsilon(nS)$ suppression at the LHC~\cite{Ferreiro:2018wbd}. It can be seen as an effective approach to deal with quarkonium suppression, accounting for the Landau damping -- the pair gets broken by a scattering with a gluon -- and the colour rotation -- a scattering with a gluon turns the pair into a colour-octet state which cannot hadronise any more. Predictions in other approaches are expected to yield similar suppressions. Given the foreseen accuracy of $\Upsilon(nS)$ measurements, the \AFTER\ program will allow one to verify such predictions in a completely new energy domain.





==> physics-high-x/buffer <==

\subsection{High-$x$ frontier for particle and astroparticle physics}
\label{section:High-x}


The purpose of this section is to address the question whether a modern fixed-target
experiment with a record energy and with high luminosities can help answer
problems at the frontier of particle and astroparticle physics.
%
We divide this section in three parts for which the physics cases are quite distinct.
In the first part, we discuss the impact of such an experiment on our understanding of the
high-$x$ structure of nucleons.
In the second part, the physics case for the high-$x$ structure of complex nuclei is
considered.
Finally, the third part is devoted to astroparticle-physics applications.

\input{physics-high-x/physics-high-x_nucleon.tex}

\input{physics-high-x/physics-high-x_nuclear.tex}

\input{physics-high-x/physics-high-x_astro.tex}





==> physics-spin/buffer <==
 \subsection{Spin physics}
\label{section:Spin-Physics}


This section focuses on the case for spin physics at \AFTER, which is very competitive in the worldwide context. 
It can be divided into two parts. 
The first relies on the use of a polarised target to carry out many SSA measurements of common probes with a high precision, but also to measure --for the first time-- 
SSA on rare perturbative probes which would remain unaccessible otherwise\footnote{Let us recall that in this c.m.s. energy range RHIC offers significantly lower luminosities with a limited access to the high $x$ in the polarised nucleons.}. 
As such, \AFTER opens a novel domain of investigation of the Sivers-like effects for several years, in order to eventually access and (indirectly) constrain the OAM of the gluons and quarks in the proton, but also in the neutron and the deuteron.
Such a quest of measuring the parton OAM goes along with a complete tridimensional tomography of the momenta of the partons confined in hadrons.

The second part of the spin physics case bears on the very large luminosities to be accumulated thanks to the fixed-target mode, combined with an acceptance towards low transverse momenta at high $x$ in the target. 
This allows one to probe in a systematic way a class of azimuthal asymmetries related to the violation of the Lam-Tung relation~\cite{Lam:1980uc} in DY production, and potentially~\cite{Lambertsen:2016wgj} to the Boer-Mulders effect~\cite{Boer:1997nt}. 
\AFTER also allows one to study its counterpart in the gluon sector, with probably the first systematic measurement of the distribution of the linearly-polarised gluons in unpolarised nucleons at large momentum fractions.

SSAs can be described by nonperturbative twist-2 TMD matrix elements and nonperturbative twist-3 collinear matrix elements (CT3) in different kinematic regions: the TMD picture holds when there are two separate scales (such as the transverse momentum $q_T$ and the invariant mass $M$ of the lepton pair in DY production with $\lqcd\leq q_T<M$), whereas the CT3 picture holds when one single hard scale is present (such as the transverse momentum $p_T$ of a pion produced in hadronic collisions with $\lqcd< p_T$). 
Both nonperturbative descriptions can in general be related in the overlapping kinematic region in $q_T$ by means of coefficients which are perturbatively calculable (see e.g.~\cite{Bacchetta:2008xw,Bacchetta:2019qkv} for some caveats in this respect). 
Both twist-2 TMD and twist-3 collinear matrix element contain essential information on the spin structure of the nucleon and their knowledge is intertwined.
\AFTER will test with high precision whether these two formalisms offer the right description of SSAs.

We first discuss the (target) STSAs (\ie\ $A_N\equiv A_{UT}$), both for quark-induced and gluon-induced processes, which give access to both quark and gluon Sivers functions and several 3-parton correlation functions.
Then we present the prospects for the measurement of spin-related azimuthal asymmetries in unpolarised hadron collisions, which also probe either the quark or the gluon content of the nucleon.
Besides the discussion of spin and azimuthal asymmetries, we also elaborate on the relation between the TMDs that can be constrained by \AFTER\ and the OAM.
Next we discuss the use of ultraperipheral collisions to access GPDs through exclusive photoproduction processes and quarkonium production.
Finally we discuss the possibility to constrain the strange-quark-helicity distribution at large $x$ through $\Lambda$ production.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Quark Sivers effect}
\label{ss:quark_sivers}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{physics-spin/physics-spin_1-quark-sivers.tex}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Gluon Sivers effect}
\label{ss:gluon_sivers}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{physics-spin/physics-spin_2-gluon-sivers.tex}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Quark-induced azimuthal asymmetries}
\label{ss:quark_BM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{physics-spin/physics-spin_3-quark-BM.tex}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Gluon-induced azimuthal asymmetries}
\label{ss:gluon_BM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{physics-spin/physics-spin_4-gluon-BM.tex}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{From TMD PDFs to the partonic orbital angular momentum}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{physics-spin/physics-spin_5-OAM.tex}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Ultraperipheral collisions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{physics-spin/physics-spin_6-UPC.tex}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Accessing the strange quark-helicity densities at high $x$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{physics-spin/physics-spin_7-StrangePDF.tex}









==> summary/buffer <==
\section{Conclusions}
\label{sec:conclusion}

Unlike the Fermilab-Tevatron and DESY-HERA colliders (with proton beams in the TeV range), no fixed-target program was planned for the LHC. In this review, we have put forward a strong physics case for such a program both for the multi-TeV proton and ion LHC beams. Such a physics case relies on extensive theory work and projection studies which have been performed with LHCb and ALICE-like detectors allowing for high precision studies in the backward hemisphere of $pp$, $pA$ and $AA$ collisions. 

These projections cover the 3 main research axes of the physics case, namely that of the nucleon and nucleus structure at high momentum fractions, that of the nucleon-spin decomposition in terms of the partonic degrees of freedom and that of the properties of the nuclear matter at extreme conditions such as those resulting from ultra-relativistic heavy-ion collisions. 

They are relevant for different possible implementations which we have reviewed including the state-of-the-art solutions provided by modern polarised gas targets or by splitting the beam with a bent crystal. For each of the possible implementations, we have also detailed the expected luminosities compatible with the LHCb and ALICE detector capabilities. For a number of studies where such projections are not yet available, we have collected the existing theory predictions for \eg\ cross sections, spin and azimuthal asymmetries or nuclear modification factors. 

Overall, we believe that the present review constitutes a very solid basis for the elaboration of a rich and fruitful LHC fixed-target program starting as early as 2020.



